DNBP: Differentiable Nonparametric Belief Propagation

We present a differentiable approach to learn the probabilistic factors used for inference by a nonparametric belief propagation algorithm. Existing nonparametric belief propagation methods rely on domain-specific features encoded in the probabilistic factors of a graphical model. In this work, we replace each crafted factor with a differentiable neural network enabling the factors to be learned using an efficient optimization routine from labeled data. By combining differentiable neural networks with an efficient belief propagation algorithm, our method learns to maintain a set of marginal posterior samples using end-to-end training. We evaluate our differentiable nonparametric belief propagation (DNBP) method on a set of articulated pose tracking tasks and compare performance with learned baselines. Results from these experiments demonstrate the effectiveness of using learned factors for tracking and suggest the practical advantage over hand-crafted approaches. The project webpage is available at: https://progress.eecs.umich.edu/projects/dnbp/ .

==> sections/impact.tex <==
\section{Probabilistic Inference for Society}




Robotics - our robot will not be able to see most of its environment when operating at the building or city scale. They can't assume the world is static, fully observable or modeled in closed form. Robots will need to maintain belief to account for these cases over long or mid-duration time frames. NNs limited by short timeframe. Generative prob inference allows the robot to maintain beliefs about the world. How can these models be brought together.

Three motivating scenarios: generalized object permanence for robotics, distributed heterogeneous inference platforms for high-dimensional continuous spaces with multimodal distributions, 

motivating requirements: Generalized object perm for rob, distributed inf for multimodal..., some way to introspect the inference process

[trusting only the NN output is a bad idea (case of robert williams) provide inferences over distributions with multiple explanations over what is perceived as a way to explain what could be possible] Characterizing model failure, to avoid predictable errors. 1) If we cant predict error. 2) If we can't predict the modes of failure (how the model will fail). Characterize the way the model fails. We want our models to generate explanations of why the model produced what it did.
